Tests of Lorentz Invariance

Lorentz invariance is a fundamental symmetry of both Einstein's theory of general relativity and quantum field theory. However, deviations from Lorentz invariance at energies approaching the Planck scale are predicted in many quantum gravity theories seeking to unify the force of gravity with the other three fundamental forces of matter. Even though any violations of Lorentz invariance are expected to be very small at observable energies, they can increase with energy and accumulate to detectable levels over large distances. Astrophysical observations involving high-energy emissions and long baselines can therefore offer exceptionally sensitive tests of Lorentz invariance. With the extreme features of astrophysical phenomena, it is possible to effectively search for signatures of Lorentz invariance violations (LIV) in the photon sector, such as vacuum dispersion, vacuum birefringence, photon decay, and photon splitting. All of these potential signatures have been studied carefully using different methods over the past few decades. This chapter attempts to review the status of our current knowledge and understanding of LIV, with particular emphasis on a summary of various astrophysical tests that have been used to set lower limits on the LIV energy scales.

==> PaxHeader/author.tex <==
30 mtime=1615114610.728470581

